A remark of Ruzsa's construction of an infinite Sidon set

A Sidon set is a set of the positive integers such that the sums of two pairs is not repeated. I. Ruzsa gave a probabilistic construction of an infinite Sidon set. In this work we present the details of a simplified proof of this construction as suggested in a paper of I. Ruzsa and J. Cilleruelo (Real and -padic Sidon sequences, Acta Sci. Math (Szeged) 70 (2004), 505-510).

==> 0222543.tex <==
%auto-ignore
